Symmetric compatibility of theta structures, with applications to change of level and isogenies

Let $m,n,d >1$ be integers such that $n=md$ and let $(B, \mathscr{M}, \Theta\_{\mathscr{M}})$ be a marked abelian variety of level $m$ over a field of odd characteristic. We study the theta structures of level $n$ for $\mathscr{M}^d$, and the theta structures on the abelian varieties $d$-isogenous to $B$, which are compatible with $\Theta\_{\mathscr{M}}$. When $d$ is odd and coprime to $m$, they correspond to the isotropic subgroups of $B[n]$, and this correspondence underlies the known algorithms in theta coordinates. In general, this is no longer true. We introduce the notion of symmetric compatibility of a torsion point with a symmetric level subgroup, and we show that a subgroup of $B[n]$ isomorphic to $(\mathbb{Z}/n\mathbb{Z})^g$ comes from a compatible theta structure if and only if it is isotropic and all its points are symmetric compatible. We extend to every $d$ Mumford's notion of compatible pairs of theta structures, defined by Mumford for $d=2$, and prove that it is equivalent to our notion, which can be tested on theta coordinates; we also describe exactly the remaining ambiguity, which explains the sign choices met when the duplication formula is used to change the level. As applications, we obtain change of level and isogeny algorithms without assuming that $d$ is odd and coprime to $m$, using $O(n^{3g} \log(d))$ and $O(n^{2g} \log(d))$ operations in the base field respectively. In particular, they give change of level algorithms for even $d$, and $2$-isogenies in level $4$ theta coordinates with an explicit control of the theta structure of the codomain.

==> def.tex <==
% vim: foldmethod=marker:foldmarker=<<<,>>>:syntax=tex

\makeatletter
\RequirePackage{mathtools} %charge amsmath (amssymb charge amsfonts)
\RequirePackage{centernot} %\centernot\mid fait un (nondiv) plus centré que \not\mid
\RequirePackage{etoolbox}

\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
% Abréviations <<<1
%\newcommand{\definedby}{\ensuremath{\coloneqq}} %:= (défini dans psfonts txfonts)
%\newcommand{\definedby}{:=} %:=
\newcommand{\defby}{\coloneqq}
\newcommand{\transp}[1]{\prescript{t}{}{#1}}

\long\def\red#1{\textcolor{red}{#1}}
\newcommand{\sgood}{\mathfrak{G}}
\newcommand{\sfcompat}{\mathfrak{C}}
\newcommand{\gtf}{\mathfrak{F}}
\newcommand{\gbar}{\overline{g}}
\newcommand{\psigz}{\psi_{g_0}}
\newcommand{\lambdazei}{\lambda^z_{e_i}}
\newcommand{\lambdaz}{\lambda^z}
\newcommand{\gzfei}{g_f^z(e_i)}
\newcommand{\tildede}{\widetilde{d'e}^\Thetabpol}
\newcommand{\tildemde}{\widetilde{-d'e}^\Thetabpol}
\newcommand{\tgzfei}{\tilde{g}_f^z(e_i)}
\newcommand{\tgzfej}{\tilde{g}_f^z(e_j)}
\newcommand{\tgzfeij}{\tilde{g}_f^z(e_i+e_j)}
\newcommand{\tGBb}{\tilde{G}_{\mathcal{B}}}
\newcommand{\gfeij}{g_f(e_i + e_j)}
\newcommand{\tgfeij}{\tilde{g}_f(e_i + e_j)}
\newcommand{\gfei}{g_f(e_i)}
\newcommand{\tgfei}{\tilde{g}_f(e_i)}
\newcommand{\tgfej}{\tilde{g}_f(e_j)}
\newcommand{\Deltam}{\Delta(m)}
\newcommand{\Deltambar}{\overline{\Delta}(m)}
\newcommand{\Deltanbar}{\overline{\Delta}(n)}
\newcommand{\otimesbpol}{\otimes_{j=1}^r [a_j]^*(\bpol)}
\newcommand{\otimespol}{\otimes_{j=1}^r [a_j]^*(\pol)}
\newcommand{\edij}{\epsilon_{d,([a_j])}}
\newcommand{\ea}{\epsilon_{[a]}}
\newcommand{\eaj}{\epsilon_{[(a_j)]}}
\newcommand{\eajs}{\epsilon_{[a_j]}}
\newcommand{\psidij}{\psi(\bpol^d, (a_j))}
\newcommand{\gpsidij}{g_{\psi_{\bpol^d,(a_j)}}}
\newcommand{\polaj}{\otimes_{j=1}^r [a_j]^*(\pol)}
\newcommand{\polajp}{\otimes_{j=1}^r [a_j]^*(\polp)}
\newcommand{\bpolaj}{\otimes_{j=1}^r [a_j]^*(\bpol)}
\newcommand{\Thetabpoldij}{\Theta_{\bpolaj}}
\newcommand{\Thetabpoldijdel}{\Theta^{\Delta}_{\bpolaj}}

\newcommand{\Thetapolalpha}{{\Thetapol^{\alpha}}}
\newcommand{\Thetapoldij}{\Theta_{\polaj}}
\newcommand{\Thetaubpoldij}{\Theta^1_{\bpolaj}}
\newcommand{\Thetaupoldij}{\Theta^1_{\polaj}}
\newcommand{\Thetadbpoldij}{\Theta^2_{\bpolaj}}

\newcommand{\gi}{{g_{-1}}}
\newcommand{\psimb}{\psi_{\mB}}
\newcommand{\psimbz}{\psi_{\mB_0}}
\newcommand{\psii}{{\psi_{-1}}}
\newcommand{\Autg}{\mathscr{G}}
\newcommand{\expo}{\epsilon}
\newcommand{\inv}{\mathrm{Inv}}
\newcommand{\invd}{\mathfrak{I}}
\newcommand{\Sinv}{{S_{inv}}}
\newcommand{\thetaact}{\mathrm{ThetaAct}}
\newcommand{\scalmult}{\mathrm{ScalarMult}}
\newcommand{\normadd}{\mathrm{NormalAdd}}
\newcommand{\diffadd}{\mathrm{DiffAdd}}
\newcommand{\compadd}{\mathrm{CompatAdd}}
\newcommand{\threeway}{\mathrm{ThreeWayAdd}}
\newcommand{\pg}{{P_{G}}}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mfr}{\mathfrak} %lettres gothiques
\newcommand{\mcal}{\mathcal}
\newcommand{\mscr}{\mathscr}

% Ensembles
% Certains paquets/classes définissent \C => stratégie: on \providecommand
% les ensembles à une lettre, eg \C, et on newcommand la version à deux
% lettres, eg \CC
\providecommand{\N}{\ensuremath{\mbb{N}}}
\newcommand{\NN}{\ensuremath{\mbb{N}}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\Aff}{\mathbb{A}}
\newcommand{\projf}{\mathrm{Proj}}
\newcommand{\Nstar}{\ensuremath{\mbb{N}^{\ast}}}
\providecommand{\Z}{\ensuremath{\mbb{Z}}}
\newcommand{\Zstar}{\ensuremath{\mbb{Z}^{\ast}}}
\providecommand{\Q}{\ensuremath{\mbb{Q}}}
\newcommand{\QQ}{\ensuremath{\mbb{Q}}}
\newcommand{\Qbar}{\overline{\Q}}
\newcommand{\Qstar}{\ensuremath{\mbb{Q}^{\ast}}}
\providecommand{\R}{\ensuremath{\mbb{R}}}
\newcommand{\RR}{\ensuremath{\mbb{R}}}
\newcommand{\Rstar}{\ensuremath{\mbb{R}^{\ast}}}
\providecommand{\C}{\ensuremath{\mbb{C}}}
\newcommand{\CC}{\ensuremath{\mbb{C}}}
\newcommand{\Cstar}{\ensuremath{\mbb{C}^{\ast}}}
\newcommand{\Un}{\ensuremath{\mbb{U}}}
\newcommand{\Kbb}{\ensuremath{\bb{K}}}
\newcommand{\Kbbstar}{\ensuremath{\mbb{K}^{\ast}}}
\newcommand{\Kstar}{\ensuremath{{K}^{\ast}}}
\newcommand{\univAb}{\mathscr{A}}
\newcommand{\poluniv}{{\pol_{\univAb}}}
\newcommand{\Thetapoluniv}{{\Theta_{\poluniv}}}
\newcommand{\Modu}{\mathbb{M}}
\newcommand{\bModu}{\overline{\mathbb{M}}}

\newcommand{\tildeG}{\widetilde{G}}
\newcommand{\tildefz}{\widetilde{f(z)}}
\newcommand{\Zz}{\mathcal{Z}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\vR}{\mathcal{R}}
\newcommand{\vx}{\overline{x}}
\newcommand{\vi}{\overline{i}}
\newcommand{\vg}{\overline{g}}
\newcommand{\qGn}{{\overline{G}(n)^4}}
\newcommand{\hGn}{{\overline{G}(n)^8}}
\newcommand{\Riem}{\mathcal{R}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\ZZn}{\Z/n\Z}
\newcommand{\xg}{\mathbb{G}}
\newcommand{\overpsi}{\bar{\psi}}
\newcommand{\chipsi}{{\chi_{\overpsi}}}
\newcommand{\kstar}{\ensuremath{k^{\ast}}}
\newcommand{\kbar}{\overline{k}}
\newcommand{\kbarstar}{{\overline{k}^{\ast}}}
\newcommand{\F}{\ensuremath{\mbb{F}}}
\newcommand{\FF}{\ensuremath{\mbb{F}}}
\newcommand{\Fstar}{\ensuremath{{\mbb{F}^\ast}}}
\newcommand{\Fq}{\ensuremath{{\mbb{F}_{q}}}}
\newcommand{\Fqn}{\ensuremath{{\mbb{F}_{q^n}}}}
\newcommand{\Fqd}{\ensuremath{{\mbb{F}_{q^d}}}}
\newcommand{\Fqdbar}{{\overline{\F}_{q^d}}}
\newcommand{\Fqstar}{{\Fq^\ast}}
\newcommand{\Fpstar}{{\Fp^\ast}}
\newcommand{\Fbar}{\overline{\F}}
\newcommand{\Fqbar}{{\overline{\F}_{q}}}
\newcommand{\Fp}{{\ensuremath{\F_{\!p}}}}
\newcommand{\Fpbar}{{\ensuremath{\overline{\F}_{\!p}}}}
\newcommand{\Pvar}{\ensuremath{\mbb{P}}}
\newcommand{\Avar}{\ensuremath{\mbb{A}}}
\newcommand{\Qp}{{\Q_p}}
\newcommand{\Qq}{{\Q_q}}
\newcommand{\stsheaf}{\mathscr{O}}
\newcommand{\polp}{{\mathscr{L}'}}
\newcommand{\polC}{{\mathscr{L}_C}}
\newcommand{\pol}{\mathscr{L}}
\newcommand{\bpol}{\mathscr{M}}
\newcommand{\hatg}{\hat{g}}
\newcommand{\hatA}{\hat{A}}
\newcommand{\hatf}{\hat{f}}
\newcommand{\hatK}{\hat{K}}
\newcommand{\hate}{\hat{e}}
\newcommand{\de}{\hat{e}}
\newcommand{\duj}{\hat{j}}
\newcommand{\hatei}{{\hat{e}_i}}
\newcommand{\tildeg}{\widetilde{g}}
\newcommand{\tildef}{\widetilde{f}}
\newcommand{\tildez}{\widetilde{z}}
\newcommand{\tildex}{\widetilde{x}}
\newcommand{\tildexthetapol}{\widetilde{x}^\Thetapol}
\newcommand{\tildexthetabpol}{\widetilde{x}^\Thetabpol}
\newcommand{\tildey}{\widetilde{y}}
\newcommand{\tildee}{{\widetilde{g}_f(e)}}
\newcommand{\tildedei}{{\widetilde{g}_f(d'e_i)}}
\newcommand{\tildedpei}{{\widetilde{g'}_f(d'e_i)}}
\newcommand{\tildeh}{\widetilde{h}}
\newcommand{\tildehatK}{\widetilde{\hat{K}}}
\newcommand{\tildeH}{\widetilde{H}}
\newcommand{\tildeZ}{\widetilde{Z}}
\newcommand{\tildeP}{\widetilde{P}}
\newcommand{\tildeQ}{\widetilde{Q}}
\newcommand{\tildexy}{\widetilde{x+y}}
\newcommand{\tildexmy}{\widetilde{x-y}}
\newcommand{\tildexpydel}{\widetilde{x+y}^{\Delta}}
\newcommand{\tildexpy}{\widetilde{x+y}}
\newcommand{\tildenullpol}{\widetilde{0}_\Thetapol}
\newcommand{\nullpol}{{0}_\Thetapol}
\newcommand{\tildenullbpol}{\widetilde{0}_\Thetabpol}
\newcommand{\nullbpol}{0_\Thetabpol}
\newcommand{\Kpol}{K(\pol)}
\newcommand{\epol}{{e_\pol}}
\newcommand{\dc}{\hat{c}}
\newcommand{\Zn}{Z(n)}
\newcommand{\drho}{\hat{\rho}}
\newcommand{\dZn}{\hat{Z}(n)}
\newcommand{\dZm}{\hat{Z}(m)}
\newcommand{\dZ}{\hat{Z}}
\newcommand{\dmu}{\hat{\mu}}
\newcommand{\dnu}{\hat{\nu}}
\newcommand{\dalpha}{\hat{\alpha}}
\newcommand{\Kn}{{K(n)}}
\newcommand{\Thetapol}{{\Theta_\pol}}
\newcommand{\Thetapold}{{\Theta_{\pol^d}}}
\newcommand{\Thetapoltwo}{{\Theta_{\pol^2}}}
\newcommand{\Thetappol}{{\Theta'_\pol}}
\newcommand{\Thetabpol}{{\Theta_\bpol}}
\newcommand{\Thetabpolp}{{\Theta'_\bpol}}
\newcommand{\Thetabpoldel}{{\Theta^{\Delta}_\bpol}}

\newcommand{\Thetapolp}{{\Theta_\polp}}
\newcommand{\Thetapolpdel}{{\Theta^{\Delta}_\polp}}

\newcommand{\Thetappolp}{{\Theta'_\polp}}
\newcommand{\Thetadpolp}{{\Theta^{\Delta}_\polp}}

\newcommand{\Thetaalphapold}{{\Theta^{\alpha}_{\pol^d}}}
\newcommand{\Thetabpold}{{\Theta_{\bpol^d}}}
\newcommand{\Thetaubpol}{{\Theta^1_\bpol}}
\newcommand{\Thetaubpold}{{\Theta^1_{\bpol^d}}}
\newcommand{\Thetadbpold}{{\Theta^2_{\bpol^d}}}
\newcommand{\Thetaalphabpold}{{\Theta^{\alpha}_{\bpol^d}}}
\newcommand{\Thetaalphapol}{{\Theta^{\alpha}_{\pol}}}


\newcommand{\Thetaupol}{{\Theta^1_\pol}}
\newcommand{\Thetadpol}{{\Theta^2_\pol}}

\newcommand{\Thetaupold}{{\Theta^1_{\pol^d}}}
    
\newcommand{\Thetapbpol}{{\Theta'_\bpol}}
\newcommand{\Thetapolbar}{{\overline{\Theta}_\pol}}
\newcommand{\Thetaupolbar}{{\overline{\Theta}^1_\pol}}
\newcommand{\Thetaalphapolbar}{{\overline{\Theta}^\alpha_\pol}}
\newcommand{\Thetappolbar}{{\overline{\Theta}'_\pol}}
\newcommand{\Thetabpolbar}{{\overline{\Theta}_\bpol}}
\newcommand{\Thetabpolpbar}{{\overline{\Theta}'_\bpol}}
\newcommand{\Thetabpoldelbar}{{\overline{\Theta}^{\Delta}_\bpol}}

\newcommand{\Thetabpoldbar}{{\overline{\Theta}_{\bpol^d}}}
\newcommand{\Thetabpoldijbar}{{\overline{\Theta}_{\otimes_{j=1}^r [a_j]^*(\bpol)}}}
\newcommand{\Thetaubpoldijbar}{{\overline{\Theta}^1_{\otimes_{j=1}^r [a_j]^*(\bpol)}}}

\newcommand{\Thetaubpolbar}{{\overline{\Theta}^1_\bpol}}
\newcommand{\Thetaubpoldbar}{{\overline{\Theta}}^1_{\bpol^d}}

\newcommand{\Gpol}{G(\pol)}
\newcommand{\pigpol}{{\pi_{\Gpol}}}
\newcommand{\pigbpol}{{\pi_{G(\bpol)}}}
\newcommand{\gabpol}{G([a]^*(\bpol))}
\newcommand{\abpol}{[a]^*(\bpol)}

\newcommand{\pifzgpol}{{\pi_{G(f_0^*(\pol))}}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\subG}{\mathfrak{G}}
\newcommand{\subzG}{{\mathfrak{G}_0}}
\newcommand{\Auts}{\mathrm{Aut_s}}
\newcommand{\Spol}{{\overline{\Theta}_\pol}}
\newcommand{\Sbpol}{{\overline{\Theta}_\bpol}}
\newcommand{\Gbpol}{G(\bpol)}
\newcommand{\Gspol}{{G^*(\pol)}}
\newcommand{\overk}{\bar{k}}
\newcommand{\barx}{\bar{x}}
\newcommand{\tildeK}{\widetilde{K}}
\newcommand{\fsharp}{{f^{\sharp}}}
%relations sur les ensembles
\newcommand{\sub}{\ensuremath{\subset}}
\newcommand{\nsub}{\ensuremath{\not\sub}}
\newcommand{\subeq}{\ensuremath{\subseteq}}
\newcommand{\subeqq}{\ensuremath{\subseteqq}}
\newcommand{\nsubeq}{\ensuremath{\nsubseteq}}
\newcommand{\subneq}{\ensuremath{\varsubsetneq}}
\newcommand{\subneqq}{\ensuremath{\subsetneqq}}
%varsubsetneqq rajoute un barré sur la barre du \sub
\providecommand{\sups}{\ensuremath{\supset}}
\newcommand{\nsups}{\ensuremath{\not\sup}}
\newcommand{\supseq}{\ensuremath{\supseteq}}
\newcommand{\nsupseq}{\ensuremath{\nsupseteq}}
\newcommand{\supsneq}{\ensuremath{\varsupsetneq}}
\newcommand{\supsneqq}{\ensuremath{\supsetneqq}}

\renewcommand*{\emptyset}{\varnothing}
\newcommand{\inter}{\ensuremath{\bigcap}}
\newcommand{\union}{\ensuremath{\bigcup}}
\newcommand{\uniondisj}{\ensuremath{\bigsqcup}}
\newcommand{\uniond}{\uniondisj}
\newcommand{\setdiff}{\backslash}
\newcommand{\symdiff}{\triangle}
\newcommand{\Jx}{{J_{\xtheta}}}
\newcommand{\vjz}{{V_J^0}}
\newcommand{\vjxz}{{V_{\Jx}^0}}
\newcommand{\xtheta}{{x_{\Thetabpol}}}
%QUESTION améliorer?
%\newcommand{\res}{\ensuremath{|}}
\newcommand{\res}[1]{\ensuremath{|_{#1}}}
%\renewcommand{\bar}{\overline}
\newcommand{\conj}{\overline}

%fait des <= , >= bien plus jolis
\let\leqhoriz\leq
\let\geqhoriz\geq
\let\leq\leqslant
\let\geq\geqslant

\newcommand{\mono}{\ensuremath{\hookrightarrow}}
\newcommand{\epi}{\ensuremath{\twoheadrightarrow}}

\newcommand{\aeq}{\ensuremath{\thickapprox}} %deux ~ verticaux (approx-equal)
\newcommand{\qeq}{\ensuremath{\cong}}        % = + ~ (quasi-equal)
\newcommand{\nqeq}{\ensuremath{\ncong}}
\newcommand{\iso}{\ensuremath{\simeq}}      % _ + ~
\newcommand{\fliso}{\ensuremath{\overset\sim\to}}      % _ + ~
%\newcommand{\niso}{\ensuremath{\not \simeq}}
\newcommand{\niso}{\ensuremath{\nsimeq}}
\newcommand{\impl}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\eqv}{\ensuremath{\Leftrightarrow}\xspace}
%sim et nsim pour les relations d'équivalences ~
%equiv : = + _ 

\newcommand{\tens}{\otimes}
\newcommand{\sommetens}{\oplus}
\newcommand{\bigtens}{\bigotimes}
\newcommand{\bigsommetens}{\bigoplus}

%groupes
\newcommand{\Ze}{\mathcal{Z}}
\newcommand{\semidir}{\rtimes}
\newcommand{\distingue}{\vartriangleleft}

\newcommand{\congr}[2]{\equiv #1 \pmod{#2}}

% délimiteurs
% \abs, \abs* pour avoir les \left\lvert..., \abs[Big] pour \Big...
\@ifpackageloaded{mathtools}{%
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\card{\lvert}{\rvert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\lnorm}{\ensuremath{\lVert}}
\newcommand{\rnorm}{\ensuremath{\rVert}}
\DeclarePairedDelimiter\norm{\lnorm}{\rnorm}
\DeclarePairedDelimiter\gen{\langle}{\rangle}
}{
\newcommand{\card}[1]{\ensuremath{\left|} #1 \ensuremath{\right|}}
\newcommand{\abs}[1]{\ensuremath{\left|} #1 \ensuremath{\right|}}
\newcommand{\norm}[1]{\lnorm #1 \rnorm} 
\newcommand{\gen}[1]{\ensuremath{\langle} #1 \ensuremath{\rangle}}
}

\newcommand{\laction}{\ensuremath{\circlearrowright}}
\newcommand{\raction}{\ensuremath{\curvearrowleft}}
\let\action\laction
\newcommand{\prodscal}[2]{\ensuremath{\left( #1 \left|#2 \right.\right)}}
%\newcommand{\prodscal}[2]{\ensuremath{\left( #1 |#2 \right)}}
\newcommand{\prodscale}[2]{\ensuremath{\left<} #1 , #2 \ensuremath{\right>}}

\newcommand{\binomial}{\binom}
\newcommand{\twovect}[2]{%
    \begin{pmatrix}
    #1 \\%
    #2%
    \end{pmatrix}%
}
\newcommand{\jacobi}[2]{\left(\dfrac{#1}{#2}\right)}
%\newcommand{\jacobi}[2]{\genfrac(){}{}{#1}{#2}}
%dfrac: display frac, tfrac: text frac, frac: automatic; cf http://tex.stackexchange.com/questions/135389/what-is-the-difference-between-dfrac-and-frac

%\newcommand{\div}{\mid}
\newcommand{\notmid}{\centernot\mid}
\newcommand{\divis}{\mid}
\newcommand{\ndivis}{\nmid}

% Operators <<<1
\newcommand{\DeclareMyOperator}[1]{%
  \expandafter\DeclareMathOperator\csname #1\endcsname{#1}
}
\newcommand{\DeclareMathOperators}{\forcsvlist{\DeclareMyOperator}}

\DeclareMathOperators{ord,sng,Card,rank,Hom,Ker,End,Aut,Sym,Alt,id,Id,lcm,pgcd,ppcm,argch,argsh,argth,Math,GL,Gl,Sp,SL,Sl,PGL,PSL,SO,SU,PSU,Spec,Var,Proj,Jac,Gal,Div,PDiv,Pic,Ext,Tor,Cl,Tr}

\DeclareMathOperator*{\limp}{\varprojlim} % Limites projective
\DeclareMathOperator*{\limi}{\varinjlim} % Limites injectives
\DeclareMathOperator{\im}{Im} %\Im fait un I bizarre
\DeclareMathOperator{\re}{Re} %\Re fait un R bizarre
\DeclareMathOperator{\Mm}{M}
\DeclareMathOperator{\Or}{O}
\DeclareMathOperator{\Uu}{U}
\newcommand{\Pico}{{\Pic_{0}}}
\DeclareMathOperator{\DEG}{deg}
\DeclareMathOperator{\car}{char}
\DeclareMathOperator{\carfr}{car}
%\DeclareMathOperator{\char}{char}

% Les flèches \vers et \depuis <<<1
%% TODO: use xparse
% \vers = \rightarrow en mode math, \longrightarrow en mode displaymath
% \vers^f = flèche étiquetée f, avec la bonne longueur
% Pour \depuis, c'est la même chose avec des flèches vers la gauche.

\newcommand{\sidispl@y}[2]{\mathchoice{#1}{#2}{#2}{#2}}%
%\def\if@empty#1#2#3{%
%  \def\@tempa{#1}%
%  \ifx\@tempa\@empty#2\else#3\fi%
%}

% From Everett Howe: Bars over math symbols  <<<1
% I think that \bar{.} gives too short a bar, and \overline{.}
% gives something which usually sticks out too far to the left,
% because of the italic slant.  Here's something that seems to
% work better, in my opinion.  The idea is to put an overline
% over an invisible roman version of the math character, and 
% put the italicized math character under that overline. --- EWH.
\newcommand{\mybar}[1]{
  \mathchoice
  {#1\llap{$\overline{\phantom{\displaystyle\rm#1}}$}}
  {#1\llap{$\overline{\phantom{\textstyle\rm#1}}$}}
  {#1\llap{$\overline{\phantom{\scriptstyle\rm#1}}$}}
  {#1\llap{$\overline{\phantom{\scriptscriptstyle\rm#1}}$}}
}  
\renewcommand{\bar}{\mybar}
\makeatother


==> packages.tex <==
% vim: foldmethod=marker:foldmarker=<<<,>>>:syntax=tex
\makeatletter
\usepackage[norelsize,linesnumbered,algoruled]{algorithm2e}
\let\oldnl\nl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}
\RequirePackage{scalerel}
\RequirePackage{etoolbox,ifluatex,ifxetex}
\providetoggle{bl@utf8}\providetoggle{bl@article}
\providetoggle{bl@babel}\providetoggle{bl@morepackages}
\toggletrue{bl@article}
\toggletrue{bl@morepackages}

\ifboolexpr{bool{luatex} or bool{xetex}} {\toggletrue{bl@utf8}}{}
\@ifclassloaded{beamer}{\togglefalse{bl@article}}{}

\iftoggle{bl@utf8}{
  \RequirePackage{fontspec}
  \RequirePackage{unicode-math}
}{
  \RequirePackage[T1]{fontenc}
  \ifluatex\RequirePackage[utf8]{luainputenc}\else\RequirePackage[utf8]{inputenc}\fi
  \RequirePackage{lmodern}
  \RequirePackage{amssymb,mathrsfs}
}
\IfFileExists{my_latex_settings}{\input{my_latex_settings}}{}

%Standard Packages
\RequirePackage{microtype}
\RequirePackage{amsmath,mathtools,yhmath}%empheq
\iftoggle{bl@article}{\RequirePackage{amsthm,thmtools}}{}
\PassOptionsToPackage{x11names,svgnames,dvipsnames}{xcolor}\RequirePackage{xcolor}
\RequirePackage{graphicx,booktabs}% tabularx/tabu
\RequirePackage{hyperref,bookmark}% varioref, pdfpages
\PassOptionsToPackage{capitalize,noabbrev}{cleveref}\RequirePackage{cleveref}
\PassOptionsToPackage{style=numeric}{biblatex} %backend=biber is default now
\RequirePackage{biblatex}

% If needed <<<
\iftoggle{bl@morepackages}{%
  \RequirePackage{iflang}
  \PassOptionsToPackage{english}{babel}\RequirePackage{babel}
  \PassOptionsToPackage{autostyle=true}{csquotes}\RequirePackage{csquotes}
  \PassOptionsToPackage{a4paper,scale=0.75}{geometry}\RequirePackage{geometry}
  \RequirePackage{tikz}
  \usetikzlibrary{arrows,chains,matrix,shapes.multipart,shapes.misc,positioning,calc,scopes,mindmap,backgrounds,fit}

  \iftoggle{bl@utf8}{}{
  \RequirePackage{eurosym}% for \euro
  \RequirePackage{textcomp}%for \textdegree
  \DeclareUnicodeCharacter{C2B0}{\textdegree}
  \DeclareUnicodeCharacter{20AC}{\ifmmode\textup{\euro}\else\euro\fi}
  }

  \iftoggle{bl@article}{%
  \PassOptionsToPackage{bottom,stable,multiple}{footmisc}\RequirePackage{footmisc}
  \RequirePackage{newfloat,caption,enumitem} %for algorithms: newfloat for \DeclareFloatingEnvironment, and caption+enumitem to set it up
  }{}
}{}

% Even more:
%\RequirePackage{xspace,glossaries}
%\RequirePackage[algoruled,onelanguage,linesnumbered]{algorithm2e}
%\RequirePackage{longtable,tabu}% if needed
% >>>
\makeatother

